Training VAEs Under Structured Residuals

Variational auto-encoders (VAEs) are a popular and powerful deep generative model. Previous works on VAEs have assumed a factorized likelihood model, whereby the output uncertainty of each pixel is assumed to be independent. This approximation is clearly limited as demonstrated by observing a residual image from a VAE reconstruction, which often possess a high level of structure. This paper demonstrates a novel scheme to incorporate a structured Gaussian likelihood prediction network within the VAE that allows the residual correlations to be modeled. Our novel architecture, with minimal increase in complexity, incorporates the covariance matrix prediction within the VAE. We also propose a new mechanism for allowing structured uncertainty on color images. Furthermore, we provide a scheme for effectively training this model, and include some suggestions for improving performance in terms of efficiency or modeling longer range correlations.

==> figures/celeba_grey_reconstructions.tex <==
\def\plotw{0.15\linewidth}

% The images to show on each column
\def\1img{9}
\def\2img{11}
\def\3img{3}
\def\4img{13}

\begin{figure}[t!]%[btph]
	\centering
%	\setlength{\tabcolsep}{2pt} % Reduce spacing between the column
	\begin{tabular}{ccccc}
	{\small Input } & \multicolumn{2}{c}{VAE} & \multicolumn{2}{c}{Ours} \\
	 & $\bmu$ & $\bmu + \epsilon$ & $\bmu$ & $\bmu + \epsilon$ \\
	\includegraphics[width=\plotw]{img/celeba_grey/recons_fig/input/\1img} &
	\includegraphics[width=\plotw]{img/celeba_grey/recons_fig/diag/recons/\1img} &
	\includegraphics[width=\plotw]{img/celeba_grey/recons_fig/diag/recons_with_residual/\1img} &
	\includegraphics[width=\plotw]{img/celeba_grey/recons_fig/covar/recons/\1img} &
	\includegraphics[width=\plotw]{img/celeba_grey/recons_fig/covar/recons_with_residual/\1img} \\
	\includegraphics[width=\plotw]{img/celeba_grey/recons_fig/input/\2img} &
	\includegraphics[width=\plotw]{img/celeba_grey/recons_fig/diag/recons/\2img} &
	\includegraphics[width=\plotw]{img/celeba_grey/recons_fig/diag/recons_with_residual/\2img} &
	\includegraphics[width=\plotw]{img/celeba_grey/recons_fig/covar/recons/\2img} &
	\includegraphics[width=\plotw]{img/celeba_grey/recons_fig/covar/recons_with_residual/\2img} \\
	\includegraphics[width=\plotw]{img/celeba_grey/recons_fig/input/\3img} &
	\includegraphics[width=\plotw]{img/celeba_grey/recons_fig/diag/recons/\3img} &
	\includegraphics[width=\plotw]{img/celeba_grey/recons_fig/diag/recons_with_residual/\3img} &
	\includegraphics[width=\plotw]{img/celeba_grey/recons_fig/covar/recons/\3img} &
	\includegraphics[width=\plotw]{img/celeba_grey/recons_fig/covar/recons_with_residual/\3img}
	\end{tabular}
	\caption{Comparison of image reconstructions for the different models.}
	\label{fig:celeba_grey_reconstructions}
\end{figure}


==> figures/celeba_grey_samples.tex <==
\def\plotw{0.15\linewidth}

% The images to show on each column
\def\1img{4}
\def\2img{5}
\def\3img{6}

\begin{figure}[t!]%[btph]
	\centering
%	\setlength{\tabcolsep}{2pt} % Reduce spacing between the column
	\begin{tabular}{cccc}
	\multicolumn{2}{c}{VAE} & \multicolumn{2}{c}{Ours} \\
	$\bmu$ & $\bmu + \epsilon$ & $\bmu$ & $\bmu + \epsilon$ \\
	\includegraphics[width=\plotw]{img/celeba_grey/samples_fig/diag/sample/\1img} &
	\includegraphics[width=\plotw]{img/celeba_grey/samples_fig/diag/sample_with_residual/\1img} &
	\includegraphics[width=\plotw]{img/celeba_grey/samples_fig/covar/sample/\1img} &
	\includegraphics[width=\plotw]{img/celeba_grey/samples_fig/covar/sample_with_residual/\1img} \\
	\includegraphics[width=\plotw]{img/celeba_grey/samples_fig/diag/sample/\2img} &
	\includegraphics[width=\plotw]{img/celeba_grey/samples_fig/diag/sample_with_residual/\2img} &
	\includegraphics[width=\plotw]{img/celeba_grey/samples_fig/covar/sample/\2img} &
	\includegraphics[width=\plotw]{img/celeba_grey/samples_fig/covar/sample_with_residual/\2img} \\
	\includegraphics[width=\plotw]{img/celeba_grey/samples_fig/diag/sample/\3img} &
	\includegraphics[width=\plotw]{img/celeba_grey/samples_fig/diag/sample_with_residual/\3img} &
	\includegraphics[width=\plotw]{img/celeba_grey/samples_fig/covar/sample/\3img} &
	\includegraphics[width=\plotw]{img/celeba_grey/samples_fig/covar/sample_with_residual/\3img}
	\end{tabular}
	\caption{ Samples drawn from our model.}
	\label{fig:celeba_grey_samples}
\end{figure}

==> figures/celeba_reconstructions_rgb.tex <==
\def\plotw{0.1\linewidth}

% The images to show on each column
\def\1img{9}
\def\2img{11}
\def\3img{3}
\def\4img{13}

\begin{figure}[t!]%[btph]
	\centering
	\setlength{\tabcolsep}{2pt} % Reduce spacing between the column
	\begin{tabular}{ccccccccc}
	{\small Input } & \multicolumn{2}{c}{VAE (Sph)} & \multicolumn{2}{c}{VAE (Diag)} & \multicolumn{2}{c}{$\beta$-VAE (Diag)} & \multicolumn{2}{c}{Ours} \\
	 & $\bmu$ & $\bmu + \epsilon$ & $\bmu$ & $\bmu + \epsilon$ & $\bmu$ & $\bmu + \epsilon$ & $\bmu$ & $\bmu + \epsilon$ \\
	\includegraphics[width=\plotw]{img/celeba/recons_fig/input/\1img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/sph/recons/\1img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/sph/recons_with_residual/\1img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/diag/recons/\1img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/diag/recons_with_residual/\1img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/beta_30_diag/recons/\1img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/beta_30_diag/recons_with_residual/\1img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/covar/recons/\1img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/covar/recons_with_residual/\1img} \\
	\includegraphics[width=\plotw]{img/celeba/recons_fig/input/\2img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/sph/recons/\2img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/sph/recons_with_residual/\2img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/diag/recons/\2img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/diag/recons_with_residual/\2img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/beta_30_diag/recons/\2img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/beta_30_diag/recons_with_residual/\2img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/covar/recons/\2img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/covar/recons_with_residual/\2img} \\
	\includegraphics[width=\plotw]{img/celeba/recons_fig/input/\3img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/sph/recons/\3img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/sph/recons_with_residual/\3img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/diag/recons/\3img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/diag/recons_with_residual/\3img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/beta_30_diag/recons/\3img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/beta_30_diag/recons_with_residual/\3img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/covar/recons/\3img} &
	\includegraphics[width=\plotw]{img/celeba/recons_fig/covar/recons_with_residual/\3img}
	\end{tabular}
	\caption{Comparison of image reconstructions for the different models.
	In contrast to previous work, our model is able to learn structured residuals.}
	\label{fig:celeba_reconstructions}
\end{figure}


==> figures/celeba_reconstructions_ycbcr_vs_rgb.tex <==
\def\plotw{0.12\linewidth}

% The images to show on each column
\def\1img{2}
\def\2img{8}
\def\3img{3}
\def\4img{13}

\begin{figure}[t!]%[btph]
	\centering
%	\setlength{\tabcolsep}{2pt} % Reduce spacing between the column
	\begin{tabular}{ccccc}
	{\small Input } & \multicolumn{2}{c}{VAE} & \multicolumn{2}{c}{VAE-YCbCr}\\
	 & $\bmu$ & $\bmu + \epsilon$ & $\bmu$ & $\bmu + \epsilon$ \\
	\includegraphics[width=\plotw]{img/celeba/diag_ycbcr_fig/input/\1img} &
	\includegraphics[width=\plotw]{img/celeba/diag_ycbcr_fig/diag_rgb/recons/\1img} &
	\includegraphics[width=\plotw]{img/celeba/diag_ycbcr_fig/diag_rgb/recons_with_residual/\1img} &
	\includegraphics[width=\plotw]{img/celeba/diag_ycbcr_fig/diag_ycbcr/recons/\1img} &
	\includegraphics[width=\plotw]{img/celeba/diag_ycbcr_fig/diag_ycbcr/recons_with_residual/\1img} \\
	\includegraphics[width=\plotw]{img/celeba/diag_ycbcr_fig/input/\2img} &
	\includegraphics[width=\plotw]{img/celeba/diag_ycbcr_fig/diag_rgb/recons/\2img} &
	\includegraphics[width=\plotw]{img/celeba/diag_ycbcr_fig/diag_rgb/recons_with_residual/\2img} &
	\includegraphics[width=\plotw]{img/celeba/diag_ycbcr_fig/diag_ycbcr/recons/\2img} &
	\includegraphics[width=\plotw]{img/celeba/diag_ycbcr_fig/diag_ycbcr/recons_with_residual/\2img} \\
	\includegraphics[width=\plotw]{img/celeba/diag_ycbcr_fig/input/\3img} &
	\includegraphics[width=\plotw]{img/celeba/diag_ycbcr_fig/diag_rgb/recons/\3img} &
	\includegraphics[width=\plotw]{img/celeba/diag_ycbcr_fig/diag_rgb/recons_with_residual/\3img} &
	\includegraphics[width=\plotw]{img/celeba/diag_ycbcr_fig/diag_ycbcr/recons/\3img} &
	\includegraphics[width=\plotw]{img/celeba/diag_ycbcr_fig/diag_ycbcr/recons_with_residual/\3img}
	\end{tabular}
	\caption{Comparison of image reconstructions for the different models.}
	\label{fig:celeba_reconstructions_ycbcr}
\end{figure}


==> figures/celeba_samples_interpolation.tex <==
\def\plotw{0.19\linewidth}
\def\ploti{3} % 1, 2, or 3 to change examples

\begin{figure}[t!]%[btph]
	\centering
	\setlength{\tabcolsep}{1pt} % Reduce spacing between the column
	\begin{tabular}{cccc}
	\includegraphics[width=\plotw]{img/celeba_grey/recons_fig/input/\1img} &
%	\includegraphics[width=\plotw]{img/celeba/interp_fig\ploti/input_source/0} &
%	\includegraphics[width=\plotw]{img/celeba/interp_fig\ploti/recons_with/0} &
%	\includegraphics[width=\plotw]{img/celeba/interp_fig\ploti/recons_with/2} &
%	\includegraphics[width=\plotw]{img/celeba/interp_fig\ploti/recons_with/4} \\
	\end{tabular}
	\caption{ Interpolations on the latent space.}
	\label{fig:celeba_samples_interpolation}
\end{figure}

==> figures/celeba_samples_rgb.tex <==
\def\plotw{0.1\linewidth}

% The images to show on each column
\def\1img{0}
\def\2img{2}
\def\3img{4}

\begin{figure}[t!]%[btph]
	\centering
	\setlength{\tabcolsep}{2pt} % Reduce spacing between the column
	\begin{tabular}{cccccccc}
	\multicolumn{2}{c}{VAE (Sph)} & \multicolumn{2}{c}{VAE (Diag)} & \multicolumn{2}{c}{$\beta$-VAE (Diag)} & \multicolumn{2}{c}{Ours} \\
	$\bmu$ & $\bmu + \epsilon$ &  $\bmu$ & $\bmu + \epsilon$ & $\bmu$ & $\bmu + \epsilon$ & $\bmu$ & $\bmu + \epsilon$ \\
	\includegraphics[width=\plotw]{img/celeba/samples_fig/sph/sample/\1img} &
	\includegraphics[width=\plotw]{img/celeba/samples_fig/sph/sample_with_residual/\1img} &
	\includegraphics[width=\plotw]{img/celeba/samples_fig/diag/sample/\1img} &
	\includegraphics[width=\plotw]{img/celeba/samples_fig/diag/sample_with_residual/\1img} &
	\includegraphics[width=\plotw]{img/celeba/samples_fig/beta_30_diag/sample/\1img} &
	\includegraphics[width=\plotw]{img/celeba/samples_fig/beta_30_diag/sample_with_residual/\1img} &
	\includegraphics[width=\plotw]{img/celeba/samples_fig/covar/sample/\1img} &
	\includegraphics[width=\plotw]{img/celeba/samples_fig/covar/sample_with_residual/\1img} \\
	\includegraphics[width=\plotw]{img/celeba/samples_fig/sph/sample/\2img} &
	\includegraphics[width=\plotw]{img/celeba/samples_fig/sph/sample_with_residual/\2img} &
	\includegraphics[width=\plotw]{img/celeba/samples_fig/diag/sample/\2img} &
	\includegraphics[width=\plotw]{img/celeba/samples_fig/diag/sample_with_residual/\2img} &
	\includegraphics[width=\plotw]{img/celeba/samples_fig/beta_30_diag/sample/\2img} &
	\includegraphics[width=\plotw]{img/celeba/samples_fig/beta_30_diag/sample_with_residual/\2img} &
	\includegraphics[width=\plotw]{img/celeba/samples_fig/covar/sample/\2img} &
	\includegraphics[width=\plotw]{img/celeba/samples_fig/covar/sample_with_residual/\2img} \\
	\includegraphics[width=\plotw]{img/celeba/samples_fig/sph/sample/\3img} &
	\includegraphics[width=\plotw]{img/celeba/samples_fig/sph/sample_with_residual/\3img} &
	\includegraphics[width=\plotw]{img/celeba/samples_fig/diag/sample/\3img} &
	\includegraphics[width=\plotw]{img/celeba/samples_fig/diag/sample_with_residual/\3img} &
	\includegraphics[width=\plotw]{img/celeba/samples_fig/beta_30_diag/sample/\3img} &
	\includegraphics[width=\plotw]{img/celeba/samples_fig/beta_30_diag/sample_with_residual/\3img} &
	\includegraphics[width=\plotw]{img/celeba/samples_fig/covar/sample/\3img} &
	\includegraphics[width=\plotw]{img/celeba/samples_fig/covar/sample_with_residual/\3img}
	\end{tabular}
	\caption{ Samples for all models, where our method is the only able to include high-frequency details such as wrinkles.}
	\label{fig:celeba_samples}
\end{figure}

==> figures/lsun_mse_error_table.tex <==
\begin{table}[t!]
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabularx}{\linewidth}{YY}
	%\toprule
	\textbf{Model} & \textbf{MSE} \\ \midrule
	VAE (Sph)~\cite{Kingma2014VAE}  & $545 \pm 286$ \\ \midrule 
	VAE (Diag)~\cite{Kingma2014VAE}  & $704 \pm 324$ \\ \midrule 
	$\beta$-VAE (Diag)~\cite{Higgins2017BVAE}  & $960 \pm 400$  \\ \midrule 
	Ours & $695 \pm 309$ \\ \bottomrule
\end{tabularx} \vspace{1pt}
\caption{Quantitative comparison of density estimation error measured as the mean squared error (MSE) on the LSUN dataset, lower is better.
}
\label{tb:lsun_error_table}
\end{table}

% VAE (sph) 544.9442138671875+-268.037841796875
% VAE (sph) YCbCr 566.5442504882812+-285.85943603515625
% VAE 704.1649169921875+-324.3963317871094
% Beta 960.0667724609375+-399.90606689453125
% Ours 694.95947265625+-308.8580627441406

==> figures/lsun_reconstructions_rgb.tex <==
\def\plotw{0.1\linewidth}

% The images to show on each column
\def\1img{9}
\def\2img{11}
\def\3img{3}
\def\4img{13}

\begin{figure}[t!]%[btph]
	\centering
	\setlength{\tabcolsep}{2pt} % Reduce spacing between the column
	\begin{tabular}{ccccccccc}
	{\small Input } & \multicolumn{2}{c}{VAE (Sph)} & \multicolumn{2}{c}{VAE (Diag)} & \multicolumn{2}{c}{$\beta$-VAE (Diag)} & \multicolumn{2}{c}{Ours} \\
	 & $\bmu$ & $\bmu + \epsilon$ & $\bmu$ & $\bmu + \epsilon$ & $\bmu$ & $\bmu + \epsilon$ & $\bmu$ & $\bmu + \epsilon$  \\
	\includegraphics[width=\plotw]{img/lsun/recons_fig/input/\1img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/sph/recons/\1img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/sph/recons_with_residual/\1img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/diag/recons/\1img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/diag/recons_with_residual/\1img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/beta_30_diag/recons/\1img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/beta_30_diag/recons_with_residual/\1img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/covar/recons/\1img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/covar/recons_with_residual/\1img} \\
	\includegraphics[width=\plotw]{img/lsun/recons_fig/input/\2img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/sph/recons/\2img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/sph/recons_with_residual/\2img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/diag/recons/\2img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/diag/recons_with_residual/\2img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/beta_30_diag/recons/\2img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/beta_30_diag/recons_with_residual/\2img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/covar/recons/\2img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/covar/recons_with_residual/\2img} \\
	\includegraphics[width=\plotw]{img/lsun/recons_fig/input/\3img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/sph/recons/\3img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/sph/recons_with_residual/\3img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/diag/recons/\3img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/diag/recons_with_residual/\3img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/beta_30_diag/recons/\3img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/beta_30_diag/recons_with_residual/\3img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/covar/recons/\3img} &
	\includegraphics[width=\plotw]{img/lsun/recons_fig/covar/recons_with_residual/\3img}
	\end{tabular}
	\caption{Comparison of image reconstructions for the different models.
	Our model is able to improve over the oversmoothed images generated by previous work.}
	\label{fig:lsun_reconstructions}
\end{figure}


==> figures/lsun_samples_rgb.tex <==
\def\plotw{0.1\linewidth}

% The images to show on each column
\def\1img{3}
\def\2img{1}
\def\3img{0}

\begin{figure}[t!]%[btph]
	\centering
	\setlength{\tabcolsep}{2pt} % Reduce spacing between the column
	\begin{tabular}{cccccccc}
	\multicolumn{2}{c}{VAE (Sph)} & \multicolumn{2}{c}{VAE (Diag)} & \multicolumn{2}{c}{$\beta$-VAE (Diag)} & \multicolumn{2}{c}{Ours} \\
	$\bmu$ & $\bmu + \epsilon$ & $\bmu$ & $\bmu + \epsilon$ & $\bmu$ & $\bmu + \epsilon$ & $\bmu$ & $\bmu + \epsilon$  \\
	\includegraphics[width=\plotw]{img/lsun/samples_fig/sph/sample/\1img} &
	\includegraphics[width=\plotw]{img/lsun/samples_fig/sph/sample_with_residual/\1img} &
	\includegraphics[width=\plotw]{img/lsun/samples_fig/diag/sample/8} &
	\includegraphics[width=\plotw]{img/lsun/samples_fig/diag/sample_with_residual/8} &
	\includegraphics[width=\plotw]{img/lsun/samples_fig/beta_30_diag/sample/\1img} &
	\includegraphics[width=\plotw]{img/lsun/samples_fig/beta_30_diag/sample_with_residual/\1img} &
	\includegraphics[width=\plotw]{img/lsun/samples_fig/covar/sample/\1img} &
	\includegraphics[width=\plotw]{img/lsun/samples_fig/covar/sample_with_residual/\1img} \\
	\includegraphics[width=\plotw]{img/lsun/samples_fig/sph/sample/\2img} &
	\includegraphics[width=\plotw]{img/lsun/samples_fig/sph/sample_with_residual/\2img} &
	\includegraphics[width=\plotw]{img/lsun/samples_fig/diag/sample/10} &
	\includegraphics[width=\plotw]{img/lsun/samples_fig/diag/sample_with_residual/10} &
	\includegraphics[width=\plotw]{img/lsun/samples_fig/beta_30_diag/sample/\2img} &
	\includegraphics[width=\plotw]{img/lsun/samples_fig/beta_30_diag/sample_with_residual/\2img} &
	\includegraphics[width=\plotw]{img/lsun/samples_fig/covar/sample/\2img} &
	\includegraphics[width=\plotw]{img/lsun/samples_fig/covar/sample_with_residual/\2img} \\
	\includegraphics[width=\plotw]{img/lsun/samples_fig/sph/sample/\3img} &
	\includegraphics[width=\plotw]{img/lsun/samples_fig/sph/sample_with_residual/\3img} &
	\includegraphics[width=\plotw]{img/lsun/samples_fig/diag/sample/14} &
	\includegraphics[width=\plotw]{img/lsun/samples_fig/diag/sample_with_residual/14} &
	\includegraphics[width=\plotw]{img/lsun/samples_fig/beta_30_diag/sample/\3img} &
	\includegraphics[width=\plotw]{img/lsun/samples_fig/beta_30_diag/sample_with_residual/\3img} &
	\includegraphics[width=\plotw]{img/lsun/samples_fig/covar/sample/\3img} &
	\includegraphics[width=\plotw]{img/lsun/samples_fig/covar/sample_with_residual/\3img}
	\end{tabular}
	\caption{ Samples drawn from the models.
	VAE fails to learn an useful latent space and $\beta$-VAE produces blurrier images than our model.}
	\label{fig:lsun_samples}
\end{figure}
